Spin-Symmetry Projected constrained Unrestricted Hartree-Fock

We introduce an electronic structure approach for spin symmetry breaking and restoration from the mean-field level. The spin-projected constrained-unrestricted Hartree-Fock (SPcUHF) method restores the broken spin symmetry inherent in spin-constrained-UHF determinants by employing a non-orthogonal Configuration Interaction (NOCI) projection method. This method includes all possible configurations in spin space compatible with a Clebsch-Gordon recoupling scheme in a NOCI calculation. The tunable one-pair-at-a-time characteristics of the symmetry-breaking process in c-UHF allow us to reduce the computational costs of full projection. SPcUHF is tested on 4-, 6-, and 8-electron systems that exhibit dominant static and/or dynamic correlations.

==> extras.tex <==
%%########################################################################
The initial step is to identify the range of all possible spin expectation values $\langle S^2\rangle$ a c-UHF can carry. The process of continuous spin-symmetry breaking starts at the $\langle S^2\rangle=0$ RHF solution, where there is no symmetry breaking and the spin-up and spin-down spatial orbitals are identical, and ends when all of the spin-up and spin-down spatial orbitals are unpaired. This range is dependent only on the number of electrons in the system $N$  \cite{cassam2015spin}

\begin{equation}
    \langle \textrm{c-UHF}| S^2|\textrm{c-UHF}\rangle \in[0,\tfrac{N}{2}].
\end{equation}
%%

c-UHF allows us to follow the symmetry-breaking process from start to finish and we can produce $\textrm{c-UHF}(S)$ where $\langle \textrm{c-UHF}| S^2|\textrm{c-UHF}\rangle \in[0,\tfrac{N}{2}]$. We later show that the c-UHF starts unpairing the spin-up and spin-down spin-orbitals one at a time, starting from the valance pair.  For those $|\textrm{c-UHF}(S)\rangle$ throughout the symmetry-breaking process where there are still paired $\alpha$ and $\beta$ spin-orbitals between spin-up and down sectors, performing spin flips can result in having identical spin-orbitals within a single spin sector, causing some determinants in the NOCI wavefunction to vanish. For instance in the four-electron example, if electrons 0 and 1 are paired and occupy the same spatial orbitals, two of the projected configurations, \(a_{0\su}^\dag a_{1\su}^\dag a_{2\sd}^\dag a_{3\sd}^\dag |\theta\rangle\) and \(a_{0\sd}^\dag a_{1\sd}^\dag a_{2\su}^\dag a_{3\su}^\dag |\theta\rangle\), vanish because identical spin-orbitals (0 and 1) are placed in the same spin sector. Additionally, determinants such as \(a_{0\su}^\dag a_{1\sd}^\dag a_{2\su}^\dag a_{3\sd}^\dag |\theta\rangle\) and \(a_{0\sd}^\dag a_{1\su}^\dag a_{2\su}^\dag a_{3\sd}^\dag |\theta\rangle\) become equivalent; flipping the degenerate spin-orbitals does not change the determinant, causing one of them to vanish. The same is true for \(a_{0\sd}^\dag a_{1\su}^\dag a_{2\sd}^\dag a_{3\su}^\dag |\theta\rangle\) and \(a_{0\su}^\dag a_{1\sd}^\dag a_{2\sd}^\dag a_{3\su}^\dag |\theta\rangle\). As a result, the calculation simplifies to a NOCI(2), retaining only the determinants \(a_{0\su}^\dag a_{1\sd}^\dag a_{2\su}^\dag a_{3\sd}^\dag |\theta\rangle\) and \(a_{0\su}^\dag a_{1\sd}^\dag a_{2\sd}^\dag a_{3\su}^\dag |\theta\rangle\). Therefore, for a given symmetry-broken c-UHF state \(|\textrm{c-UHF}(S)\rangle\), the number of projected configurations remaining in the NOCI basis is determined by the number of unpaired spin orbitals (\(M\)) between the two spin sectors in the system, following the binomial \(\binom{M}{M/2}\).


We are now in the position to discuss the algorithmic steps in the spin-projected c-UHF method (SPcUHF).  The goal of the SPcUHF is to compute the ground-state energy of a molecular system in a variational spirit. We apply a global variational optimization and for each constrained $\langle S^2\rangle$ we will compute a c-UHF ground-state energy $E_{\textrm{c-UHF}}(S)$, and project the associated $|\textrm{c-UHF}(S)\rangle$ state on proper spin eigenstates using the NOCI approach outlined above.  See Algorithm \ref{algo:spcuhf} for an outline in pseudocode.

\begin{algorithm}[H]
\caption{spin-projected c-UHF}\label{algo:spcuhf}
\begin{algorithmic}[1]
    \Require{$N$,$\langle S^2\rangle$}\Comment{Number of particles in the system and imposed spin expectation value}
    \Ensure{$E$}\Comment{selected energy eigenvalues}
    \Procedure{spin-projected c-UHF}{}%\Comment{The g.c.d. of a and b}
    \State $|\textrm{c-UHF}\rangle \gets$ \Call{cUHF}{N,$\langle S^2\rangle$}
    \State $k\gets \binom{N}{N/2}$ \label{algo:k}
    \State $\textrm{NOCIBasis}\amir{(k_{eff})} \gets$ \Call{GenNOCIBasis}{$k,|\textrm{cUHF}\rangle$}\Comment{\amir{$k_{eff} \gets \binom{M}{M/2}$}} %M is \# unpaired electrons} %Generate all spin configurations}
    \State $E\gets$ \Call{NOCI}{$k_{\amir{eff}}$, NOCIBasis\amir{($k_{eff}$)}}
     % \For{\texttt{<some condition>}}
    %  \State \texttt{<do stuff>}
     % \EndFor
    \EndProcedure
\end{algorithmic}
\end{algorithm}

The resulting NOCI energy $E_{\textrm{NOCI}}$ will be lower (but not strictly) than the reference c-UHF energy $E_{\textrm{c-UHF}}(S)$ because of added quantum correlations.  Finally, we retain the lowest $E_{\textrm{NOCI}}$ over all expectation values $\langle S^2\rangle$ as the variational minimum.  In all figures below, we will report energy profiles of both the c-UHF and SPcUHF/NOCI methods as a function of the imposed spin constraint $\langle S^2\rangle$, although the resulting SPcUHF states are technically free from spin contamination by construction.  The reason is to reference the imposed $\langle S^2\rangle$ that went into the seed c-UHF state.


\begin{figure}[H]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=1.0]{Be631g_NOCI}
  \caption{}
  \label{fig:Be_631g_NOCI}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=1.0]{Be_MOoverlap}
  \caption{}
  \label{fig:Be_631g_overlap}
\end{subfigure}
\caption{For Be/6-31G: (a) Comparison of c-UHF, NOCI(2), and NOCI(6) energies with FCI energy across the full range of imposed constraint $\langle S^2\rangle$. (b) The overlap between $\alpha$ (0, 2) and $\beta$ (1, 3) molecular spin orbitals.}
\label{fig:Be_631g}
\end{figure}
%%####################################################################################
